Subsampling Sparse Graphons Under Minimal Assumptions

We establish a general theory for subsampling network data generated by the sparse graphon model. In contrast to previous work for networks, we demonstrate validity under minimal assumptions; the main requirement is weak convergence of the functional of interest. We study the properties of two procedures: vertex subsampling and $p$-subsampling. For the first, we prove validity under the mild condition that the number of subsampled vertices is $o(n)$. For the second, we establish validity under analogous conditions on the expected subsample size. For both procedures, we also establish conditions under which uniform validity holds. Furthermore, under appropriate sparsity conditions, we derive limiting distributions for the nonzero eigenvalues of the adjacency matrix of a low rank sparse graphon. Our weak convergence result immediately yields the validity of subsampling for the nonzero eigenvalues under suitable assumptions.

==> real-data.tex <==
We consider the problem of testing whether two social networks are generated by the same sparse graphon.  The dataset, which first appeared in \citet{traud-social-networks-facebook}, involves Facebook friendship networks from 100 universities in 2005.  Facebook networks are well-suited for our method, as the networks are typically large and not too sparse. Friendship networks are also undirected, which ensures that the corresponding eigenvalues are real-valued.

We will consider a two-sample test based on subsampled eigenvalues for comparing social networks of different universities.  With the same Facebook dataset, \citet{Bhattacharyya-subsample-count-features} consider two-sample testing using subsampled count functionals; here, we examine the relative merits of using subsampled eigenvalue statistics for comparing two networks.  

Before proceeding, we would like to mention some of the strengths and weaknesses of the eigenvalue approach compared to the subgraph approach that are not directly related to the power of the test.  First, note that the entire spectrum of a symmetric matrix can be computed in $O(n^3)$ time and calculating the top few eigenvalues can be performed even faster.  For count functionals, a brute-force subgraph search with $p= |\mathcal{V}(R)|$ has complexity $O(n^p)$.  However, as noted in \citet{Bickel-Chen-Levina-method-of-moments}, for sparser graphs, certain functionals such as kl-wheels can be counted faster.  From a computational perspective, eigenvalue statistics generally may be preferable for network comparisons.  On the other hand, eigenvalue statistics require stronger conditions on the sparsity level; consequently, count functionals may be safer to use for sparser graphs.   

With eigenvalue statistics, it is also not clear a priori which statistics will be most effective at distinguishing two networks.  To limit false discoveries, we consider a sample splitting procedure in which one subnetwork is used for formulating hypotheses and the other is used for testing the hypotheses.  The most natural procedure under the model (\ref{bernoulli-model}) is node-splitting, in which nodes are randomly split into two disjoint sets and the corresponding induced subgraphs are used.  Under our model, the induced subgraphs are independent and thus, inferences based on node-splitting are valid. 

 Node-splitting is often criticized for being wasteful, as the edges between the induced subgraphs are discarded.  However, when the latent positions are treated as random, this is often a price that is worth paying to ensure that the two datasets are independent. While not captured in our dataset, the student body changes over time, so viewing the population as fixed may not be appropriate.    

\subsection{Exploratory Data Analysis}
We choose 20 collegiate networks to analyze; the universities considered are top liberal arts schools, public univerities, and private universities.  From each of these networks, we set aside a subnetwork for exploration.  To formulate hypotheses, we perform hierarchical clustering on the top eigenvalues calculated on the respective subnetworks.  We present results for hierarchical clustering with complete linkage under the Euclidean distance; we also tried other variants of hierarchical clustering, but the results in this section were not sensitive to the choice of clustering method. In Appendix \ref{appendix-clustering}, we also extend our clustering analysis to 40 selected collegiate networks.   

\begin{figure}[H] 
	\centering
  	\includegraphics[angle=90,clip,trim=3.4cm 0.1cm 0.1cm 0.1cm,width=0.76\linewidth]{top_50.pdf} 
  	\caption{Dendogram from hierarchical clustering on the top 50 normalized eigenvalues}
\end{figure} 

 Above, we see that he groupings suggested by hierarchical clustering coincide with the previously mentioned liberal arts, public, and private divisions.  The groups may also correspond to the size of the student body; see Appendix \ref{appendix-clustering} for further discussion.  In either case, it seems that eigenvalues, while not easily interpretable, contain salient information about the underlying graphs.  Furthermore, it seems that the performance of the clustering method is not driven by the top few eigenvalues.  Using the top 10 eigenvalues, Columbia and Cornell are placed in a similar group as the public universities, but using the top 25 or 50 eigenvalues, we see that these universities are grouped with other private universities.

Based on our clustering analysis, we decide to make the following comparisons, ordered in ascending difficulty: Berkeley vs Stanford, Penn vs Columbia, Harvard vs MIT, and Yale vs Princeton.  For each comparison, we inspect the spectra and choose a suitable test statistic on the exploration dataset.  Then, on the held-out subnetwork, we use subsampling to perform a two-sample test. 
\begin{figure}[H]
\centering 
  \begin{subfigure}[b]{0.46\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{berkeleyvstanford.pdf} 
    \vspace{0.5ex} 
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.46\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{columbiavpenn.pdf} 
    \vspace{0.5ex}
  \end{subfigure} 
  \begin{subfigure}[b]{0.46\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{harvardvmit} 
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.46\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{princetonvyale} 
  \end{subfigure} 
  \caption{A comparison of the top 25 normalized eigenvalues calculated on the subnetwork used for exploration.  We see that the behavior of the top few eigenvalues and the rate of decay of the eigenvalues are a few features that vary across collegiate networks.  While differences in the spectrum for three of the comparisons are visible to the eye, it appears that the Princeton and Yale spectra are very similar.} 
\end{figure} 

\subsection{Data Analysis Results}
Using the exploratory dataset, we construct test statistics for each of the two-sample tests. We mainly consider eigenvalues near the top of the spectrum since it appears that inference becomes more difficult for eigenvalues that are smaller in magnitude.  For each network, we construct a $97.5\%$ confidence interval for the test statistic. If the confidence intervals are disjoint, we may reject the null hypothesis that the graphs were generated by the same graphon with a significance level of $\alpha = 0.05$. The confidence intervals are constructed via vertex subsampling, with a subsample size chosen to be about $33 \%$ of the test set.  While this may seem to be a large proportion, it appears that smaller subsample sizes result in the estimated parameters being systematically outside of the confidence interval, suggesting substantial bias.  One exception is the maximum eigenvalue, which generally seems well-behaved.  

Our results are presented in the table below.  We reject the null hypothesis for the Columbia vs Penn and Harvard vs MIT comparisons, but fail to reject for the other two comparisons.  In the exploratory phase, both hierarchical clustering and the eigenvalue plots suggested that it would be difficult to distinguish between the spectra of the Yale and Princeton networks, so it is not surprising that we were not able to reject the null hypothesis here. 

\begin{table}
\renewcommand*{\arraystretch}{1.5}
\centering
\begin{tabular}{|l|l|l|l|l|l|l}
\cline{1-6}
  Schools   &   n              & Test statistic          & Value       &   $97.5\%$ CI        & Decision       &  \\ \cline{1-6}                                                                
  Berkeley  & $11468$      & $\lambda_5/n \rho_n$  &   1.336     &  $(1.164,1.347)$     & Fail to reject $\mathrm{H}_0$         &  \\
  Stanford  &  $5810$      &                       &   1.148     &  $(1.046, 1.173)$    &                      &  \\ \cline{1-6}
  Columbia  & $5885$       & $\lambda_1/n \rho_n$  &   2.522     &  $(2.124,2.769)$     & Reject $\mathrm{H}_0$         &  \\
  Penn      & $7458$       &                       &   2.033     &  $(1.853, 2.100)$    &                      &  \\ \cline{1-6}
  Harvard   & $7563$       & $\lambda_5/n \rho_n$  &   1.206     &  $(1.119, 1.250)$    & Reject $\mathrm{H}_0$         &  \\
  MIT       & $3220$       &                       &   1.060     &  $(0.944,1.071)$     &                      &  \\ \cline{1-6}
  Princeton & $3298$      & $\lambda_4/n \rho_n$  &   1.057     &  $(0.929, 1.066)$    & Fail to reject $\mathrm{H}_0$ &  \\
  Yale      & $4289$       &                       &   1.031     &  $(0.906, 1.030)$    &                      &  \\ \cline{1-6}
\end{tabular}
\smallskip
\caption{Two-sample test results} 
\end{table} 

On the other hand, exploratory data analysis suggested that the Berkeley vs Stanford comparison should perhaps be the easiest.  There are a few possible explanations for the behavior of our test.  The first is that we were unlucky with sample splitting; we chose the fifth eigenvalue based on differences in the exploration set, but this may not have been representative.  The second and third eigenvalues appear to be significantly different on the test set.  In addition, the Berkeley network is much sparser, with an average degree of $74$ compared to $98$ for Stanford, even though the network is much larger.  It may simply be the case that inference is more difficult for sparser graphs.  In addition, one of the main differences between the two networks is the rate of decay of the eigenvalues.  The approach considered here may have low power for distinguishing between graphs that differ in the tail of the spectra.  The Harvard vs MIT comparison appeared to be more difficult, but the graphs differed in the behavior of the top few eigenvalues and our test appears to have reasonable power in this case.  

Finally, we would like to emphasize that the validity of the subsampling confidence interval hinges on a weak convergence result, which requires a non-trivial sparsity condition.  Since our notion of sparsity pertains to a sequence of graphs and we only have one observation for each school, it is difficult to say whether this condition is satisfied.  However, the clustering results are promising, with sensible groupings for graphs of different sizes.  One would also expect the confidence intervals to be very wide if the graphs were too sparse, but this does not appear to be the case.  A more pressing issue is the bias.  We have taken steps to mitigate this issue, but it is also worth considering explicit bias corrections.   







